Taming Past LTL and Flat Counter Systems

Reachability and LTL model-checking problems for flat counter systems are known to be decidable but whereas the reachability problem can be shown in NP, the best known complexity upper bound for the latter problem is made of a tower of several exponentials. Herein, we show that the problem is only NP-complete even if LTL admits past-time operators and arithmetical constraints on counters. Actually, the NP upper bound is shown by adequately combining a new stuttering theorem for Past LTL and the property of small integer solutions for quantifier-free Presburger formulae. Other complexity results are proved, for instance for restricted classes of flat counter systems.

==> proof-cps-1-in-p.tex <==
\begin{proof}
Consider a path schema $\aschema=\aseg.\aloop^{\omega}$ in a counter system with only one loop $\aloop$. Due to the structure of $\aschema$ there
exists at most one run $\arun$ respecting $\aschema$ and starting from a given initial configuration $\aconf_0$. $\footprint{\arun}$ (defined in
Section \ref{section-disjunction}) is of the form $u.v^{\omega}$, which is an ultimately periodic word. Since, the only loop $\aloop$ is to be taken an
infinite number of times, we have, $\length{v}=\length{\aloop}$ which is polynomial in size of the input, but $\length{u}$ can be exponential. But,
note that $\wordof{\arun(0)\arun(1)\cdots\arun(\length{u})}\in\aseg \cdot \aloop^{+}$
 where the number of 
repetition of $\aloop$ may be an
exponential number of times. The algorithm computes the number of different possible sets of term maps (defined in Section~\ref{section-disjunction}),
that the nodes of $\aloop$ can have. At most, this can be polynomially many times due to the monotonocity of guards and 
counter constraints. Next, for
each such assignment $i$ of term maps to the nodes of $\aloop$, the algorithm calculates the number of iterations $nl_i$ of $\aloop$, for which the
terms remain in their respective term map. Note that each of these $nl_i$ can be exponentially large. Now, the formula is symbolically verified over
the ultimately periodic path where the nodes of the path schema are augmented with the term maps.
%The algorithm calculates the number of times 
%each copy of $\aloop$, with the same term maps, is repeated. Thereafter, it performs symbolic model checking on a truncated version of $\footprint{\arun}$, which by the
%stuttering theorem, is equivalent as the model checking on the original footprint.

Before defining the algorithm formally, we need to define some notions to be used in the algorithm. For a path segment 
$\aseg= \anedge_1 \anedge_2\cdots
\anedge_{\length{\aseg}}$, we define $\aseg[i,j]=\anedge_i\anedge_{i+1}\cdots \anedge_j$ for $1\leq i\leq j\leq |\aseg|$. Also, for a loop segment
$\aloop$, we say a tuple of term maps 
$(\atermmap_1,\atermmap_2,\cdots,\atermmap_{\length{\aloop}})$ is \defstyle{final} iff for every term
$\aterm=\sum_j a_j \acounter_j\in T$ and for all $1\leq i\leq \length{\aloop}$,
\begin{itemize}
  \item  $\sum_j a_j \effect{\aloop}[j]>0$ implies $\atermmap_i(\aterm)$ is maximal in $I$.%has an upperbound $\infty$
  \item  $\sum_j a_j \effect{\aloop}[j]<0$ implies $\atermmap_i(\aterm)$ is minimal in $I$.%has a lowerbound $-\infty$. 
\end{itemize}
where $\effect{\aloop}$ is as defined in Section \ref{section-path-schemas}.

%Also, note that, since there is a unique run (if any) respecting $\aschema$, we can mark the nodes of 
$\aschema$ (possibly with copying) with term-maps. 
%For a path segment $\aseg=w_1w_2\cdots w_{\length{\aseg}}$ with $w_i=(\astate_i,\aguard_i,\anupdate_i,\astate_{i+1})\in\triangle$ for $i\in[1,\length{\aseg}]$ and a tuple of term maps $a=(\atermmap_1,\atermmap_2,\cdots,\atermmap_{\length{\aseg}})$, we define $\aseg\times a=w'_1w'_2\cdots w'_{\length{aseg}}$ where $w'_i=(\pair{\alabelling(\astate_i)}{\atermmap_i}$. 
Since the unique run respecting $\aschema$ must contain $\aseg$ and copies of $\aloop$, we can specify the term maps for
$\aword=\aseg \cdot \aloop$. Consider the function 
%% $f_{\aconf} : \{0,1,2,\ldots,\length{\aword}\} \rightarrow I^{T}$ 
$\amap_{{\rm init}} : \{0,1,2,\ldots,\length{\aword}\} \rightarrow I^{T}$ 
for a given configuration
$\aconf=\pair{\astate_0}{\avect_0}$, defined as:
\begin{itemize}
\itemsep 0 cm 
  \item $\amap_{{\rm init}}(0)=\atermmap_0$ iff for each term $\aterm=\sum_j a_j \acounter_j\in T$, we have that, $\sum_j
    a_j.\avect_0[j]\in\atermmap_0(\aterm)$ and $\atermmap_0 \vdash \guard{\aword(0)}$.
  \item for $1\leq i\leq\length{\aword}$ as $\amap_{{\rm init}}(i)=\atermmap_i$ iff, for each term 
   $\aterm=\sum_j a_j \acounter_j\in T$, we have that,
    $\sum_j a_j.(\effect{\aword[1,i]}[j]+\avect_0[j])\in\atermmap_i(\aterm)$ and $\atermmap_i\vdash \guard{\aword(i)}$.
  \item Otherwise, if the term maps do not satisfy the guards, then there does not exist any run and hence 
  $\amap_{{\rm init}}(i)$ is undefined. 
\end{itemize}
Also, we consider the function $curr: T \rightarrow \rel$ which, in the algorithm, gives the value of the terms at specific positions of the run. The
function $val_{curr}:\edges^{+}\rightarrow I^{T}$, is defined as $val_{curr}(w)=\atermmap$ where for all $\aterm=\sum_j a_j \acounter_j\in T,
curr(\aterm)+\sum_j a_j.(\effect{w}[j])\in \atermmap(\aterm)$. For a path segment $\aseg=\anedge_1\anedge_2\cdots\anedge_{\length{\aseg}}$ with
$\anedge_i=(\astate_i,\aguard_i,\anupdate_i,\astate_{i+1})\in\edges$ for $i\in[1,\length{\aseg}]$ and a tuple of term maps
$a=(\atermmap_1,\atermmap_2,\cdots,\allowbreak\atermmap_{\length{\aseg}})$, we define $\aseg\times a=\anedge'_1\anedge'_2\cdots\anedge'_{\length{\aseg}}$ where
$\anedge'_i=(\pair{\astate_i}{\atermmap_i},\aguard_i,\anupdate_i,\pair{\astate_{i+1}}{\atermmap_{i+1}})$. 

Given an initial configuration $\aconf$, we calculate the term maps for each position of $\aseg$ and the first iteration of $\aloop$, using
$\amap_{{\rm init}}$. Subsequently, we calculate new tuples of term maps 
$(\atermmap_1,\atermmap_2\cdots\atermmap_{\length{\aloop}})$ for $\aloop$ and the
number of iterations $nl$ of $\aloop$ for which the terms remain in their respective term map from the tuple. We store the tuple of term maps in an
array $A$ and the number of iterations corresponding to tuple $i$ in $nl_i$. In case, at any position, we reach some term maps that does not satisfy
some guard, the procedure is aborted as it signifies that there does not exist any run. 
Note that there are polynomially many entries in $A$ but each
of the $nl_i$ can be exponential. We perform symbolic model checking over a path schema augmented with the calculated term maps. The augmented
path schema is obtained by performing $\aloop\times A[i]$ for each $i$. But the number of times $\aloop\times A[i]$ is repeated, $nl_i$ can be
exponential. Thus, instead of taking $\aloop\times A[i]$, $nl_i$ times, we take it 
$\mathtt{Min}(nl_i,2\td{\aformula} + 5)$ times. 
By Theorem~\ref{theorem-stuttering}, 
%% And by
%% Stuttering theorem (Theorem~\ref{theorem-stuttering}), 
we have that the two path schemas are equivalent in terms of satisfiability of $\aformula$. 
The polynomial-time algorithm is described in Algorithm~\ref{algorithm-cps}.

\begin{algorithm}
\caption{The \ptime \  algorithm with inputs $\aschema=\aseg \cdot \aloop^\omega$, $\aconf=\pair{\astate_0}{\avect_0}$,
$\aformula$}
\label{algorithm-cps}
\begin{algorithmic}[1]
\STATE Build a resource $\aresource = \triple{\aset}{T}{B}$ and a set of intervals $I$ coherent with $\aschema$ and $\aformula$.
\STATE Compute $\amap_{{\rm init}}(i)$ for all $i\in[0,\length{\aseg.\aloop}-1]$.
\STATE {\bf if} for some $i\in \interval{0}{\length{\aseg \cdot \aloop}-1}$, $\amap_{{\rm init}}(i)$ is undefined
       {\bf then} {\bf abort} 
%% 
%% \IF{for some $i\in[0,\length{\aseg.\aloop}-1]$, $f_{\aconf}(i)$ is undefined}
%% \STATE Abort
%% \ENDIF
%% 
%\STATE Define $\aseg'=\aformulater(1)\aformulater(2)\ldots\aformulater(\length{\aseg})$.
\STATE For each term $\aterm=\sum_j a_j \acounter_j\in T$, $curr(\aterm) :=\sum_j a_j.(\effect{\aseg \cdot \aloop}[j]+\avect_0[j])$.
%\STATE Mark each node of $\aseg$ with appropriate term-maps depending on $\aconf_0$, to construct $\aseg'\in(\powerset{\aset} \times I^T)^{\length{\aseg}}$
%\STATE Initially mark a copy of $\aloop$ with term-maps designated as $\atermmap_1,\atermmap_2\cdots\atermmap_{\length{\aloop}}$.
%\STATE Let $index =1$ and $A[index]=\atermmap_1,\atermmap_2\cdots\atermmap_{\length{\aloop}}$.
%\WHILE{$A[index]$ is not final}
\STATE $h:=1$; $A[1]:=(\amap_{{\rm init}}(\length{\aseg}),\amap_{{\rm init}}(\length{\aseg}+1)\cdots \amap_{{\rm init}}(\length{\aseg.\aloop}-1))$
%% \REPEAT
\WHILE{$A[h]$ is not final}
\STATE Compute, $nl_h=min\{nl|i\in [1,\length{\aloop}], \aterm\in T, val_{curr}(\aloop^{nl} \cdot \aloop[1,i])(\aterm)\neq A[h](i)(\aterm)\}$.
%\STATE For $j>0$, we define, $nl_j$ as the smallest integer such that, for some term $\aterm=\sum_j a_j \acounter_j\in T$ at some position
%       $i$ in $\aloop$ we have that $\sum_j a_j \vec{v}[j]\notin \atermmap(t)$ where 
%       $\vec{v}[j]=\effect{\aseg}[j]+\sum_{k\leq j}nl_k \effect{\aloop}[j] + \effect{\aloop[1,i]}[j]$ and $\atermmap=A[index](i)$.
\STATE $h:=h+1$
\STATE $A[h] :=(\atermmap_1,\atermmap_2\cdots\atermmap_{\length{\aloop}})$, 
       such that at all positions $i$ in $\aloop$ we have that $val_{curr}(\aloop^{nl_{h}} \cdot \aloop[1,i])= \atermmap_i$.
\STATE For every term $\aterm=\sum_j a_j \cdot \acounter_j\in T$, set 
       $curr(\aterm)=curr(\aterm)+\sum_j a_j.(nl_h.\effect{\aloop}[j])$.
\STATE {\bf if} there is $i\in \interval{1}{\length{\aloop}}$ such that  $A[h](i) \nvdash\guard{\aloop(i)}$
       {\bf then} {\bf abort}
\ENDWHILE
%% 
%% \STATE Abort
%% \IF{$\exists i\in [1,\length{\aloop}], A[h](i)\nvdash\guard{\aloop(i)}$}
%% \STATE Abort
%% \ENDIF
%%
%% \UNTIL{$A[h]$ is not final}
%\ENDWHILE
%\STATE Continue the last 2 steps until for every term $\aterm=\sum_j a_j \acounter_j\in T$ and every position 
%       $i$ in $\aloop$, $\sum_j a_j \effect{\aloop}[j]>0$ [resp. $\sum_j a_j \effect{\aloop}[j]<0$] implies $\atermmap_i(\aterm)$ has an upperbound 
%       $\infty$[resp. lowerbound $-\infty$].
%\STATE Let $n$ be the number of iterations of the above steps.
\STATE For $j \in \interval{1}{h-1}$, $T[j] := \mathtt{Min}(nl_j,2\td{\aformula} + 5)$ 
%% \STATE For $j \in \interval{1}{h-1}$, $trunc(nl_j) := \mathtt{Min}(nl_j,2\td{\aformula} + 5)$ 
%% \STATE For $1\leq j \leq h, trunc(nl_j) = min(nl_j,2\td{\aformula} + 5)$
\STATE Check that
$\proj((\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times A[1])^{T[1]}.(\aloop \times
A[2])^{T[2]}\ldots(\aloop\times A[h-1])^{T[h-1]}(\aloop\times A[h])^{\omega}),0 \symbmodels \aformula$
%% \STATE Check that
%% $\proj((\aseg\times(f_{\aconf}(0),\ldots,f_{\aconf}(\length{\aseg}-1)).(\aloop\times A[1])^{trunc(nl_1)}.(\aloop\times
%% A[2])^{trunc(nl_2)}\ldots(\aloop\times A[h-1])^{trunc(nl_{h-1})}(\aloop\times A[h])^{\omega}),0\symbmodels \aformula$
%\STATE Check that $\aseg'\aloop'_1\aloop'_2\ldots(\aloop'_{index})^{\omega}, 0 \symbmodels \aformula$ where,\\
%      $\aseg'=\pair{\aseg(0)}{f_{\aconf}(0)}\pair{\aseg(1)}{f_{\aconf}(1)}\ldots\pair{\aseg(\length{\aseg}-1)}{f_{\aconf}(\length{\aseg}-1)}$\\
%      $i\in[1,h], \aloop'_i=(\pair{\aloop(1)}{A[i](1)}\pair{\aloop(2)}{A[i](2)}\ldots\pair{\aloop(\length{\aloop})}{A[i](\length{\aloop})})^{trunc(nl_i)}$ 
\end{algorithmic}
\end{algorithm}
It now remains to prove that the algorithm completes in PTime and is correct.
\begin{lemma}
Algorithm \ref{algorithm-cps} terminates in time which is at most a polynomial in the size of the input.
\end{lemma}
\begin{proof}
We will verify that each step of the algorithm can be performed in polynomial time.
\begin{itemize}
  \item Building a resource and a set of intervals can be done by scanning the input once.
  \item Since the updates of $\aschema$ is part of the input, we can compute 
        $\amap_{{\rm init}}$
        %% $f_{\aconf}$ 
        for all positions in $\aseg \cdot \aloop$ in polynomial time.
  \item Calculation of $curr$ depends on the previous value of $curr$ and the coefficients appearing in the guards of $\aschema$. Hence, it involves 
        addition and multiplication of at most polynomial number of bits. Thus, this can be performed in polynomial time.
  \item The maximum possible value for $h$ is bounded by a polynomial given by Lemma~\ref{lemma-bounded-skeleton}. 
        Indeed,  the process described in the while loop is the same as the creation of unfolded path schema set 
        $Y_{\aschema}$. The only difference being that 
        there exists only one possible run, if any and hence $Y_{\aschema}$ is a singleton set.
  \item Calculation of each $nl_h$ requires computing $val_{curr}$ which again involves arithmetical operations on 
        polynomially many bits. Thus, this requires polynomial time only.
  \item Checking $(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times A[1])^{T[1]} 
       (\aloop\times A[2])^{T[2]} \ldots\allowbreak 
       (\aloop\times A[h-1])^{T[h-1]}\allowbreak(\aloop\times A[h])^\omega, 0 \symbmodels \aformula$ can be 
      done in polynomial time for the following reasons. 
    \begin{itemize}
      \item By definition of $T[h]$, size of $(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).
      (\aloop\times A[1])^{T[1]}
        (\aloop\times A[2])^{T[2]} \ldots\allowbreak (\aloop\times A[h-1])^{T[h-1]}(\aloop\times A[h])^\omega$ is
        polynomial in the size of the input.
      \item By~\cite{Laroussinie&Markey&Schnoebelen02}, 
        $(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times
        A[1])^{T[1]} (\aloop\times A[2])^{T[2]} \allowbreak \ldots (\aloop\times
        A[h-1])^{T[h-1]}\allowbreak(\aloop\times A[h])^\omega, 0 \symbmodels \aformula$ can be checked in time
        $\mathcal{O}(\sizeof{\aformula}^2 \times\allowbreak\length{\aseg \cdot \aloop^{T[1]}\allowbreak \aloop^{T[2]} \cdots
          \aloop^{T[h-1]} \aloop})$.  Indeed, $\symbmodels$ is analogous to the satisfaction relation for plain Past LTL.
     \end{itemize}
\end{itemize}
%\qed
\end{proof}

\begin{lemma}
$\aschema,\aconf\models \aformula$ iff Algorithm \ref{algorithm-cps} on inputs $\aschema,\aconf,\aformula$ has an accepting run.
\end{lemma}
\begin{proof}
Let us first assume that $\aschema,\aconf\models \aformula$. We will show that there exists a vector of positive integers 
$\vec{nL}=(nl_1,nl_2\ldots nl_h)$ for some $h\in\Nat$ such that Algorithm \ref{algorithm-cps} has an accepting run. Clearly, the 
transitions taken by a run $\arun$ respecting $\aschema$ and satisfying $\aformula$ is of the form, $\aseg\aloop^{\omega}$. This 
can be decomposed in the form $\aseg \aloop^{nl_1} \aloop^{nl_2} \ldots \aloop^{nl_h} \aloop^\omega$, depending on the portion of $\aschema$ traversed, 
such that for each consecutive 
copy of $\aloop$, the term maps associated with the nodes change. It is easy to see that this decomposition is same as the one calculated by the algorithm.
 Now, the elements of $\vec{nL}$ can be exponential. 
But due to Lemma \ref{lemma-footprint-run} and Stuttering theorem (Theorem \ref{theorem-stuttering}), we know that,
$(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times A[1])^{nl_1} 
(\aloop\times A[2])^{nl_2} \ldots 
(\aloop\times A[h-1])^{nl_{h-1}}(\aloop\times A[h])^\omega, 0 \symbmodels \aformula$ iff
$(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times A[1])^{T[1]} (\aloop\times A[2])^{T[2]} \allowbreak\ldots\allowbreak 
(\aloop\times A[h-1])^{T[h-1]}\allowbreak(\aloop\times A[h])^\omega, 0 \allowbreak\symbmodels \aformula$. Hence, 
the algorithm has an accepting run.

Now, we suppose that the algorithm has an accepting run on inputs $\aschema,\aconf$ and $\aformula$. We will prove that $\aschema,\aconf\models \aformula$.
Since the algorithm has an accepting run, we assume the integers calculated by it are $nl_1,nl_2,\cdots,nl_h$.
Let $\aword = \aseg \aloop^{nl_1} \aloop^{nl_2} \ldots \aloop^{nl_h} \aloop^\omega$ and
$\arun = \pair{\pair{\astate_0}{\atermmap_0}}{\vec{x_0}}
\pair{\pair{\astate_1}{\atermmap_1}}{\vec{x_1}} 
\pair{\pair{\astate_2}{\atermmap_2}}{\vec{x_2}} \cdots \in (\states' \times \Zed^n)^{\omega}$
be defined as follows: 
for every $i \geq 0$, $\astate_i \egdef \pi_1(\source{\aword(i)})$,
$\vec{x_0} \egdef \vec{v_0}$ and for every $i \geq 1$, we have
      $\vec{x_i} \egdef \vec{x_{i-1}} + \update{\aword(i)}$.  
By the calculation of $l_j$, $1\leq j\leq n$, in the algorithm, it is easy to check that $\pair{\astate_0}{\vec{x_0}}\pair{\astate_1}{\vec{x_1}} 
\pair{\astate_2}{\vec{x_2}} \cdots \in (\states \times \Zed^n)^{\omega}$ is a run respecting $\aschema$. Algorithm \ref{algorithm-cps} guarantees that
$(\aseg\times(\amap_{{\rm init}}(0),\ldots,\amap_{{\rm init}}(\length{\aseg}-1)).(\aloop\times A[1])^{T[1]} (\aloop\times A[2])^{T[2]} \ldots 
(\aloop\times A[h-1])^{T[h-1]}(\aloop\times A[h])^\omega, 0 \allowbreak\symbmodels \aformula$.
And thus, by Lemma~\ref{lemma-footprint-run}  and Theorem~\ref{theorem-stuttering}, we have, 
$\pair{\astate_0}{\vec{x_0}}\pair{\astate_1}{\vec{x_1}}\allowbreak\pair{\astate_2}{\vec{x_2}} \cdots ,0\symbmodels \aformula$.
\end{proof}


\end{proof}


